A Synthetic Modal Generation of Additive Manufacturing Roughness Surfaces from Images

A method to infer and synthetically extrapolate roughness fields from electron microscope scans of additively manufactured surfaces using an adaptation of Rogallo's synthetic turbulence method [R. S. Rogallo, NASA Technical Memorandum 81315, 1981] based on Fourier modes is presented. The resulting synthetic roughness fields are smooth and are compatible with grid generators in computational fluid dynamics or other numerical simulations. Unlike machine learning methods, which can require over twenty scans of surface roughness for training, the Fourier mode based method can extrapolate homogeneous synthetic roughness fields using a single physical roughness scan to any desired size and range. Five types of synthetic roughness fields are generated using an electron microscope roughness image from literature. A comparison of their spectral energy and two-point correlation spectra show that the synthetic fields closely approximate the roughness structures and spectral energy of the scan.

==> Sections/Recommendations.tex <==
\section{Recommendations}
\label{sec:Recommendations}
The main limitation of the presented method is the image data extraction procedure being solely applicable to \gls{HSV} colormap input images. The image data extraction procedure should be expanded to include the extraction of other colormaps input images, making the synthetic roughness generation process applicable to a larger adversary of \gls{AM} roughness images in literature.

Furthermore, \gls{ML} methods are still considered to be superior to the presented method in terms of synthetic roughness field generation capability, but only with a sufficient amount of training data. It would be interesting to investigate and discover what the break even point is in terms of the amount of training data necessary to outperform the presented methods with \gls{ML} methods. With this information, research groups can evaluate their resources and determine if it is more beneficial to use \gls{ML} methods or the presented method for the generation of synthetic \gls{AM} roughness for their numerical simulations.
